Policy Regularization via Noisy Advantage Values for Cooperative Multi-agent Actor-Critic methods

Recent works have applied the Proximal Policy Optimization (PPO) to the multi-agent cooperative tasks, such as Independent PPO (IPPO); and vanilla Multi-agent PPO (MAPPO) which has a centralized value function. However, previous literature shows that MAPPO may not perform as well as Independent PPO (IPPO) and the Fine-tuned QMIX on Starcraft Multi-Agent Challenge (SMAC). MAPPO-Feature-Pruned (MAPPO-FP) improves the performance of MAPPO by the carefully designed agent-specific features, which may be not friendly to algorithmic utility. By contrast, we find that MAPPO may face the problem of \textit{The Policies Overfitting in Multi-agent Cooperation(POMAC)}, as they learn policies by the sampled advantage values. Then POMAC may lead to updating the multi-agent policies in a suboptimal direction and prevent the agents from exploring better trajectories. In this paper, to mitigate the multi-agent policies overfitting, we propose a novel policy regularization method, which disturbs the advantage values via random Gaussian noise. The experimental results show that our method outperforms the Fine-tuned QMIX, MAPPO-FP, and achieves SOTA on SMAC without agent-specific features. We open-source the code at \url{https://github.com/hijkzzz/noisy-mappo}.

==> sections/proof.tex <==
\label{proof}
\begin{definition}
Original objective function:
\begin{align} 
\hat{J^{MAPPO}} &= \mathbb{E}_{\tau \sim \mathcal{D}}\left[\frac{\pi\left(\vec{a_{t}} \mid s_{t}\right)}{\pi_{{ \text { old }}}\left(\vec{a_{t}} \mid s_{t}\right)} A_{t}^{old}(s_t, \vec{a}^t)\right] \notag \\
&= \mathbb{E}_{\tau \sim \mathcal{D}}\left[\prod_i^N \frac{\pi^i\left(a_{t}^i \mid s_{t}\right)}{\pi^{i}_{old}\left(a_{t}^i \mid s_{t}\right)} A_{t}^{old}(s_t, \vec{a}^t)\right] \notag
\end{align}

Surrogate objective function:
\begin{align}
\hat{\widetilde{J^{MAPPO}}} &= \mathbb{E}_{\tau \sim \mathcal{D}}\left[\frac{1}{N} \sum_i^{N} \frac{ \pi^i\left(a_{t}^i \mid s_{t}\right)}{\pi^i_{{\text {old }}}\left(a_{t}^i \mid s_{t}\right)} A^{old}_{t}(s_t, \vec{a}^t)\right]  \notag
\end{align}

where $\mathcal{D}$ is the trajectories sampled by joint policy $\pi^{old}$; and $N$ is the number of agents.
\end{definition}

In this section, we prove that

\begin{equation}
    \mathop{maxmize}\hat{\widetilde{J^{MAPPO}}} \Rightarrow 
    \mathop{maxmize}\hat{J^{MAPPO}}
\end{equation}

holds \textbf{approximately} with a small gap (depends on the size of $\epsilon$) and following  constraints,

\begin{enumerate}
    \item Clip constraint:  $1 - \epsilon \le \frac{\pi^i(. \mid s_t)}{\pi^i_{\theta_{\mathrm{old}}}(. \mid s_t)} \le 1 + \epsilon$, where $\epsilon$ is the clip parameter; We use this constraint to approximate the KL divergence constraint.
    \item Probability constraint: $\sum_{k=1}^\mathcal{\vert K \vert} \pi^i\left(a_{t}^{i,k} \mid s_{t}\right) = 1$, where $\mathcal{K}$ denotes all actions of the agent.
\end{enumerate}

\begin{proof}
We know that that maximizing surrogate objective function $\hat{\widetilde{J^{MAPPO}}}$ is equivalent to, 

\begin{enumerate}
    \item Maximizing the invidual ratio for each agent $\frac{ \pi^i\left(a_{t}^i \mid s_{t}\right)}{\pi^i_{{\text {old }}}\left(a_{t}^i \mid s_{t}\right)}$ for each item in  $\hat{\widetilde{J^{MAPPO}}}$ that $A^{old}_t > 0$.
    \item Minimizing the invidual ratio for each agent $\frac{ \pi^i\left(a_{t}^i \mid s_{t}\right)}{\pi^i_{{\text {old }}}\left(a_{t}^i \mid s_{t}\right)}$ for each item in  $\hat{\widetilde{J^{MAPPO}}}$ that $A^{old}_t < 0$.
\end{enumerate}

and maximizing original objective function $\hat{J^{MAPPO}}$ is equivalent to, 

\begin{enumerate}
    \item Maximizing the joint ratio $\prod_i^N \frac{\pi^i\left(a_{t}^i \mid s_{t}\right)}{\pi^{i}_{old}\left(a_{t}^i \mid s_{t}\right)}$ for each item in $\hat{J^{MAPPO}}$ that $A^{old}_t > 0$.
    \item Minimizing the joint ratio $\prod_i^N \frac{\pi^i\left(a_{t}^i \mid s_{t}\right)}{\pi^{i}_{old}\left(a_{t}^i \mid s_{t}\right)}$ for each item in $\hat{J^{MAPPO}}$ that $A^{old}_t < 0$.
\end{enumerate}

Due to the probability constraint, the above problems can be equated as: \textbf{transferring the action probability of a item with advantage value $A$ to another item with advantage value $A^\prime$.}, which makes the sum of these two items larger.

Given that $\pi^* = \mathop{\arg\max}_{\pi}\hat{\widetilde{J^{MAPPO}}}$, and there exists 

\begin{align}
    \pi^{\prime} = \mathop{\arg\max}_{\pi}\hat{J^{MAPPO}} \ne \pi^* 
    \text{and }
    \hat{J^{MAPPO}}_{\pi^{\prime}} > \hat{J^{MAPPO}}_{\pi^*} \notag
\end{align}

which means that there are some action probability transfers between $\pi^*$ and $\pi^\prime$: e.g, given a pair of items with the same state $s$ and different actions $\vec{a}$ and $\vec{a^\prime}$, in the original objective function $\hat{J^{MAPPO}}_{\pi^*}$,

\begin{align}
     &\frac{\pi^{j,*}\left(a^j \mid s\right)}{\pi^{j}_{old}\left(a^j \mid s\right)} \cdot \prod_{i \ne j}^N \frac{\pi^{i, *}\left(a^i \mid s\right)}{\pi^{i}_{old}\left(a^i \mid s\right)} A^{old}(s, \vec{a}) \notag \\
     &\frac{\pi^{j,*}\left(a^{j, \prime} \mid s\right)}{\pi^{j}_{old}\left(a^{j, \prime} \mid s\right)} \cdot \prod_{i \ne j}^N \frac{\pi^{i,*}\left(a^{i, \prime} \mid s\right)}{\pi^{i}_{old}\left(a^{i, \prime} \mid s\right)} A^{old}(s, \vec{a}^\prime)
     \label{eqn:two_item}
\end{align}

$\pi^\prime$ can transfer the action probability of $\pi^{j,*}\left(a^{j, \prime} \mid s\right)$  to   $\pi^{j,*}\left(a^j \mid s\right)$ to make that $\hat{J^{MAPPO}}_{\pi^\prime} > \hat{J^{MAPPO}}_{\pi^*}$ with following conditions hold for above two items,

\begin{enumerate}
\item $\frac{A^{old}(s, \vec{a})}{\pi^{j}_{old}\left(a^j \mid s\right)} \prod_{i \ne j}^N \frac{\pi^{i, *}\left(a^i \mid s\right)}{\pi^{i}_{old}\left(a^i \mid s\right)}  > \frac{A^{old}(s, \vec{a}^\prime)}{\pi^{j}_{old}\left(a^{j, \prime} \mid s\right)} \prod_{i \ne j}^N \frac{\pi^{i,*}\left(a^{i, \prime} \mid s\right)}{\pi^{i}_{old}\left(a^{i, \prime} \mid s\right)} \label{eqn:cond1}$; this allows the transfer of probabilities to increase the size of the sum of above a pair items.

\item Clip constraint:  $ \frac{\pi^{j,*}\left(a^j \mid s\right)}{\pi^{j}_{old}\left(a^j \mid s\right)} < 1 + \epsilon$ and $\frac{\pi^{j,*}\left(a^{j,\prime} \mid s\right)}{\pi^{j, \prime}_{old}\left(a^j \mid s\right)} > 1 - \epsilon$.
\end{enumerate}

As $\pi^*$ is a optimal solution of $\hat{\widetilde{J^{MAPPO}}}_{\pi}$, we obtain that $\frac{A^{old}(s, \vec{a})}{\pi^{j}_{old}\left(a^j \mid s\right)} \le \frac{A^{old}(s, \vec{a}^\prime)}{\pi^{j}_{old}\left(a^{j, \prime} \mid s\right)}$. Since if this inequality does not hold, we can obtain that $\hat{\widetilde{J^{MAPPO}}}_{\pi^{\prime}} > \hat{\widetilde{J^{MAPPO}}}_{\pi^{*}}$ with the same action probability transfer from $\pi^{j,*}\left(a^{j, \prime} \mid s\right)$ to  $\pi^{j,*}\left(a^j \mid s\right)$, which contradicts that $\pi^{*}$ is the optimal solution of $\hat{\widetilde{J^{MAPPO}}}_{\pi}$. As we know that $\mathbb{E}_{\vec{a} \sim \pi} [A^{old}(s, \vec{a})] = 0$, and $A^{old}(s, \vec{a})$ can determine the sign of above two items (Eq. \ref{eqn:two_item}), which implies that condition (1) can only hold if $A^{old}(s, \vec{a})$ and $A^{old}(s, \vec{a}^\prime)$ have the same sign. Thus the probability of the condition (1) holds is small. 

Thus we assume that above two conditions (1) and (2) hold with \textbf{a small probability $\eta$} for a ratio item $\frac{\pi^{j,*}\left(a^j \mid s\right)}{\pi^{j}_{old}\left(a^j \mid s\right)}$ where $j \in N$. Then, $\pi^\prime$ can only transfer the actions probability of $\left| \mathcal{D}\right| \cdot N \cdot \eta$ ratio items of $\hat{J^{MAPPO}}_{\pi^*}$ to increase the size of it. Next, we can obatin that  
\begin{equation}
\frac{\left| \hat{J^{MAPPO}}_{\pi^{\prime}} \right|}{\left| \hat{J^{MAPPO}}_{\pi^*} \right|} \approx \frac{\left| \mathcal{D}\right| \cdot \left[ (1 + C)^{\eta \cdot N}\right]}{ \left| \mathcal{D} \right| \cdot 1} = (1 + C)^{\eta \cdot N} \label{eqn:gap}
\end{equation}
where $C$ is the average lift size of the ratio items in $\hat{J^{MAPPO}}_{\pi^*}$ for a pair of action probability transfer; and $C$ is a small value due to (1) $A^{old}(s, \vec{a})$ and $A^{old}(s, \vec{a}^\prime)$ have the same sign, which makes that the probability transfer to increase the size of one item while decreasing the size of the other.  (2) By the clip constraint, $C$ is limited by value of $\epsilon$. Especially, since $\pi^*$ is a optimal solution of $\hat{\widetilde{J^{MAPPO}}}_{\pi}$, it implies that most of the policy ratios are already approaching the bound of the clip limit with a small $\epsilon$.

Finally, as the small clip hyperparameter $\epsilon$ implies the $C$ are also small, \textbf{we obtain that $\pi^*$ is close to $\pi^\prime$ with a gap (Eq .\ref{eqn:gap}) when $\epsilon$ is a small value}. 
\end{proof}














